Merging Facts, Crafting Fallacies: Evaluating the Contradictory Nature of Aggregated Factual Claims in Long-Form Generations

Long-form generations from large language models (LLMs) contain a mix of factual and non-factual claims, making evaluating factuality difficult. Prior works evaluate the factuality of a long paragraph by decomposing it into multiple facts, verifying those facts independently, and aggregating the results. Such methods assume that combining factual claims forms a factual paragraph. The above assumption can be violated: we show that strong open-source models like Llama-chat can generate paragraphs that contain verifiable facts, but the facts are combined into a non-factual paragraph due to entity ambiguity. We further reveal that existing factuality metrics, including FActScore and citation recall, cannot properly evaluate these non-factual paragraphs and overestimate their factuality. To address this, we introduce an enhanced metric, D-FActScore, specifically designed for content with ambiguous entities. We evaluate the D-FActScores of people biographies generated by retrieval-augmented LLMs. We show that D-FActScore can better assess the factuality of paragraphs with entity ambiguity than FActScore. We also find that four widely used open-source LLMs tend to mix information of distinct entities to form non-factual paragraphs, making their D-FActScore much lower than FActScore by over 10%.

==> prompt.tex <==
Park Chan-wook, born on August 23, 1963, in Seoul, South Korea, is a renowned filmmaker and actor known for his impactful work in the film industry. He made his acting debut in the film "The Moon is the Sun's Dream" in 1992 and continued to appear in small and supporting roles throughout the 1990s.\\
\\
- Park Chan-wook was born on August 23, 1963.\\
- Park Chan-wook was born in Seoul, South Korea.\\
- Park Chan-wook is a renowned filmmaker.\\
- Park Chan-wook is an actor.\\
- Park Chan-wook is known for his impactful work in the film industry.\\
- He made his acting debut in the film.\\
- He made his acting debut in The Moon is the Sun's Dream.\\
- The Moon is the Sun's Dream is a film.\\
- The Moon is the Sun's Dream was released in 1992.\\
- After his acting debut, he appeared in small and supporting roles.\\
- After his acting debut, he appeared in small and supporting roles throughout the 1990s.\\
\\
- Park Chan-wook was born on August 23, 1963.\\
- Park Chan-wook was born in Seoul, South Korea.\\
- Park Chan-wook is a renowned filmmaker.\\
- Park Chan-wook is an actor.\\
- Park Chan-wook is known for his impactful work in the film industry.\\
- He made his acting debut in the film.\\
- He made his acting debut in The Moon is the Sun's Dream.\\
- The Moon is the Sun's Dream is a film.\\
- The Moon is the Sun's Dream was released in 1992.\\
- After his acting debut, he appeared in small and supporting roles.\\
- After his acting debut, he appeared in small and supporting roles throughout the 1990s.\\
\\
- Mike McCoy is an American.\\
- Mike McCoy is an American football coach.\\
- Mike McCoy has a distinguished history.\\
- Mike McCoy has a distinguished history in playing.\\
- Mike McCoy has a distinguished history in coaching.\\
- Mike McCoy has a distinguished history in the NFL.\\
- Mike McCoy has played in the NFL.\\
- Mike McCoy has coached in the NFL.\\
- McCoy played for the Broncos.\\
- McCoy played for the Broncos during his professional career.\\
- McCoy played for the San Diego Chargers.\\
- McCoy played for the San Diego Chargers during his professional career.\\
- McCoy played for the Minnesota Vikings.\\
- McCoy played for the Minnesota Vikings during his professional career.\\
- McCoy played for the Jacksonville Jaguars.\\
- McCoy played for the Jacksonville Jaguars during his professional career.\\
- He played began his journey in the world of football.\\
- He played was a quarterback at Long Beach State University.\\
- He played transferred to the University of Utah.\\
- He played continued to develop his skills at the University of Utah.\\
- He played showcased his talent at the University of Utah.\\
\\
Gavin Hamilton, born in Lanarkshire, Scotland in 1723, was a prominent neoclassical history painter and antiquarian who lived in Rome. He was also known for his role in the hunt for antiquities in the area. Gavin Hamilton, born in 1974, is an all-round cricketer who played for England in one Test and for Scotland in several One Day Internationals. Gavin Hamilton, who lived from 1561 to 1612, was the bishop of Galloway and was educated at the University of St. Andrews. Lastly, Gavin George Hamilton, born in 1872, was a Scottish Liberal politician and the 2nd Baron Hamilton of Dalzell.\\
\\
- Gavin Hamilton was born in Lanarkshire, Scotland in 1723.\\
- Gavin Hamilton was a prominent neoclassical history painter.\\
- Gavin Hamilton was a prominent antiquarian.\\
- Gavin Hamilton lived in Rome.\\
- He was known for his role.\\
- His role was in the hunt for antiquities.\\
- The hunt for antiquities was in the area.\\
- Gavin Hamilton was born in 1974.\\
- Gavin Hamilton is an all-round cricketer.\\
- Gavin Hamilton played for England in one Test.\\
- Gavin Hamilton played for Scotland in several One Day Internationals.\\
- Gavin George Hamilton was born in 1872.\\
- Gavin George Hamilton was a Scottish Liberal politician.\\
- Gavin George Hamilton was the 2nd Baron Hamilton of Dalzell.\\
\\
- Gavin Hamilton was born in Lanarkshire, Scotland in 1723.\\
- Gavin Hamilton was a prominent neoclassical history painter.\\
- Gavin Hamilton was a prominent antiquarian.\\
- Gavin Hamilton lived in Rome.\\
- He was known for his role.\\
- His role was in the hunt for antiquities.\\
- The hunt for antiquities was in the area.\\
- ===\\
- Gavin Hamilton was born in 1974.\\
- Gavin Hamilton is an all-round cricketer.\\
- Gavin Hamilton played for England in one Test.\\
- Gavin Hamilton played for Scotland in several One Day Internationals.\\
- ===\\
- Gavin George Hamilton was born in 1872.\\
- Gavin George Hamilton was a Scottish Liberal politician.\\
- Gavin George Hamilton was the 2nd Baron Hamilton of Dalzell.
